An Extension of the Character Ring of sl(3) and Its Quantisation

We construct a commutative ring with identity which extends the ring of characters of finite dimensional representations of sl(3). It is generated by characters with values in the group ring $Z[\tilde{W}]$ of the extended affine Weyl group of $\hat{sl}(3)_k$ at $k\not \in Q$. The `quantised' version at rational level $k+3=3/p$ realises the fusion rules of a WZW conformal field theory based on admissible representations of $\hat{sl}(3)_k$.

==> ch-pic.tex <==
%Date: Tue, 14 Jul 1998 13:32:20 +0200
%From: Valentina Petkova <petkova@ts.infn.it>

\input amssym.def
\input amssym.tex
%\documentclass{article}
%\usepackage{xy}
\input xy
\xyoption{all}
%\input xypic
%\input xypoly
\nopagenumbers

\def\bt{\bullet}\def\cr{\circ}\def\st{\star}\def\tm{{\rm x}}
\def\hrt{\halfrootthree}
\def\wyg{{\cal W}} \def\fwd{{\cal G}}

\def\tW{\tilde W}
\def\CC{{\cal W}^{(+)}} \def\tC{\tilde\CC} %%% chambers
\def\UU{{\cal U}}                         %%% `fiber' over w_0
\def\VV{{\cal V}}                         %%% supp of `Verma'
%\def\bG#1{{\Gamma}_{(#1)}}               %%% supp of f.d.  module
\def\GG{{\cal G}}                         %%% supp of f.d. `module'

\def\hrt{\halfrootthree} 
\input xy \xyoption{all}

\def\UNIT{\blacktriangleleft\kern-.6em\blacktriangleright}

\def\BEX#1#2 {\save\POS,c="o"="e.#1" *{#2}
            \PATH ~={**\dir{-}} 
            '"o"+(1,0)="1.#1" *{#2}' "o"+(2,1)="21.#1" *{#2}'
			'"o"+(2,2)="3.#1" *{#2}' "o"+(1,2)="12.#1" *{#2}'
			'"o"+(0,1)="2.#1" *{#2}' "o", \restore}			

\def\PEX#1#2 {\save\POS, 
         c="o"="3.#1" *{#2}   %%% *+!D{#1} 
         \PATH ~={**\dir{-}} 
         '"o"-(1,0)="12.#1" *{#2} ^{2}' "o"-(2,1)="2.#1" *{#2} ^{1}'
         '"2.#1"-(1,0)="2+.#1" *{#2} _{0}' "2.#1"  % needle
		 '"o"-(2,2)="e.#1"  *{#2} ^{2}' "o"-(1,2)="1.#1" *{#2} ^{1}
         '"1.#1"-(0,1)="1+.#1" *{#2} ^{0}' "1.#1"  % needle
		 '"o"-(0,1)="21.#1" *{#2} ^{2}' "o" ^{1}
%		 "1.#1";"1.#1"-(0,1)="1+.#1" *{#2} ^{0},
% 		 "2.#1";"2.#1"-(1,0)="2+.#1" *{#2} ^{0},
		 '"e.#1";"e.#1"-(1,1)="e+.#1" *{#2} ^{0},	 \restore}	




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% fig. 1.  picture for Cayley graph of W and chamber
\xy
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
  (0,0) ,   {\PEX {a}{\circ} },
  "e+.a",   {\PEX {b}{\bullet} },
  (-3,0),   {\PEX {c}{\circ} },
  "e+.c",   {\PEX {d}{\circ} },
  (0,-3),   {\PEX {e}{\circ} },
  "e+.e",   {\PEX {f}{\circ} },
  "e+.b",   {\PEX {g}{\bullet} },  
{  \ar @{-} "2+.g";"e+.d" _{1} }, 
{  \ar @{-} "1+.g";"e+.f" ^{2} },   
"e+.d" *{\bullet},"e.d" *{\bullet},"1.d" *{\bullet},
"e+.f" *{\bullet},"e.f" *{\bullet},"2.f" *{\bullet},
"e.a" *{\UNIT},
(1,0);(-11,-6) **@{.},(0,1);(-6,-11) **@{.},
(-4,2) %*++!DR{w_{2}(\CC)} 
;(2,-4) **@{.},
(-10,-8) *{\CC}, (1,1) *{\CC w_{121}},
(-4.5,1.5) *{\CC w_{2}},(-3.5,2.5) *{\CC w_{12}},
(1.5,-4.5) *{\CC w_{1}},(2.5,-3.5) *{\CC w_{21}},
\endxy   \bigskip
fig. 1. \quad Parts of the Cayley graph of $W$, the
chamber $\CC$ and the KW action on it. \bigskip 
\vskip 1cm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 2. picture for `fiber' U
\xy  
0;<1cm,0cm>: %<\hrt cm,-.5cm>::
(0,0) *{\UNIT} ; (0,1) *{\bullet} **\dir{-} ? *+!R{w_0}, 
(1,0)          ; (1,1) **\dir{-} ? *+!R{w_1}, 
(2,0)          ; (2,1) **\dir{-} ? *+!R{w_2}, 
(3,0)          ; (3,1) **\dir{-} ? *+!R{w_0},
(0,0);(1,0) *{\bullet} **\dir{-} ? *\dir{>} *+!U{\gamma},
(1,0);(2,0) *{\bullet} **\dir{-} ? *\dir{>} *+!U{\gamma},
(2,0);(3,0) *{\UNIT} **\dir{-} ? *\dir{>} *+!U{\gamma},
%
(0,1);(1,1) *{\bullet} **\dir{-} ? *\dir{>} *+!D{\gamma},
(1,1);(2,1) *{\bullet} **\dir{-} ? *\dir{>} *+!D{\gamma},
(2,1);(3,1) *{\bullet} **\dir{-} ? *\dir{>} *+!D{\gamma},
%
% \PATH ~={**\dir{-}} ' (1,0) *{\bullet}
\endxy \bigskip
fig. 2. \quad The set $\UU$. 
% i.e., the `fiber' in $\tW$ over the edge $w_0$. \bigskip

\vskip 1cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 3. picture for map "i"
\xy
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
(-2,-2.5);(2,-.5) **@{.},(-2.5,-2);(-.5,2) **@{.},
(-2,-2. );(2,0. ) **@{.},(-2. ,-2);(0. ,2) **@{.},
(-2,-1.5);(2,0.5) **@{.},(-1.5,-2);(0.5,2) **@{.},
(-2,-1. );(2,1. ) **@{.},(-1. ,-2);(1. ,2) **@{.}, % edges of chamber
(-4,-1.5);(4,2.5) **@{.},(-1.5,-4);(2.5,4) **@{.},
(-2, 0. );(2,2. ) **@{.},( 0. ,-2);(2. ,2) **@{.},
(-2, 0.5);(2,2.5) **@{.},( 0.5,-2);(2.5,2) **@{.},
%
(-1,3);(3,-1) **@{.},
%
  (0,0) *{\UNIT}, {\BEX {a}{\bullet} },
  (-1,-2)       , {\BEX {b}{\bullet} },
  (-2,-1)       , {\BEX {c}{\bullet} },
%
(.5,0)*!UL{1},(0,.5)*!UR{2},
%
"e.a";"e.b" **\dir{--} ? *\dir{>} *+!R{\overline{\Lambda}_2} ,  
"e.a";"e.c" **\dir{--} ? *\dir{>} *+!L{\overline{\Lambda}_1} ,  
\endxy \bigskip
fig. 3.\quad The map $\iota$. \bigskip

\vskip 1.5cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig 4. of the `adjoint'
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
(-0.5,-0.5)*{w_{1210}=t_{-\theta}},
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
 '(0,0)*+{1}*\frm{o}^1'(0,1)*+{1}*\frm{o}^2},
%
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(2,1)*+{2}*\frm{o}^2},
{(0,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,2)*+{2}*\frm{o}^1},
%
{(3,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
		 '(3,1)*+{2}*\frm{o}^2'(2,1)*+{2}*\frm{o}^0
		 '(2,2)*+{3}*\frm{o}^1'(1,2)*+{2}*\frm{o}^2
         '(1,3)*+{2}*\frm{o}^0'(0,3)*+{1}*\frm{o}^1},
%
{(3,1)*+{2}\PATH ~={**\dir{-}}'(4,2)*+{2}^1},
{(2,2)*+{3}\PATH ~={**\dir{-}}'(3,3)*+{4}^0},
{(1,3)*+{2}\PATH ~={**\dir{-}}'(2,4)*+{2}^2},
%
{(5,2)*+{1}*\frm{o}
		   \PATH ~={**\dir{-}}
		   '(4,2)*+{2}*\frm{o}^2'(4,3)*+{3}*\frm{o}^0
		   '(3,3)*+{4}*\frm{o}^1'(3,4)*+{3}*\frm{o}^2
		   '(2,4)*+{2}*\frm{o}^0'(2,5)*+{1}*\frm{o}^1},
%
{(5,2)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(6,3)*+{1}*\frm{o}^0},
{(4,3)*+{3}*\frm{o}\PATH ~={**\dir{-}}'(5,4)*+{2}*\frm{o}^2},
{(3,4)*+{3}*\frm{o}\PATH ~={**\dir{-}}'(4,5)*+{2}*\frm{o}^1},
{(2,5)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(3,6)*+{1}*\frm{o}^0},
%
{(6,3)*+{1}*\frm{o}
			  \PATH ~={**\dir{-}}
			  '(6,4)*+{1}*\frm{o}^2'(5,4)*+{2}*\frm{o}^0
			  '(5,5)*+{2}*\frm{o}^1'(4,5)*+{2}*\frm{o}^2
			  '(4,6)*+{1}*\frm{o}^0'(3,6)*+{1}*\frm{o}^1},
%
{(5,5)*+{2}\PATH ~={**\dir{-}}'(6,6)*+{1}*\frm{o}^0},
\endxy
\bigskip fig. 4 
%\medskip%\noindent
The weight diagram $\GG_{w_{1210}}$  %of the `adjoint' %[1,1] diagram 
with weight multiplicities indicated in the circles.

\vskip 1.5cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig 5. of the `Verma' at translates of origin
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
(-0.5,-0.5)*{t_{-\lambda}},
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
          '(0,0)*+{1}*\frm{o}^1'(0,1)*+{1}*\frm{o}^2},
%
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(2,1)*+{2}*\frm{o}^2},
{(0,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,2)*+{2}*\frm{o}^1},
%
{(4,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
         '(3,0)*+{1}*\frm{o}^1'(3,1)*+{2}*\frm{o}^2
         '(2,1)*+{2}*\frm{o}^0'(2,2)*+{3}*\frm{o}^1
		 '(1,2)*+{2}*\frm{o}^2'(1,3)*+{2}*\frm{o}^0
		 '(0,3)*+{1}*\frm{o}^1'(0,4)*+{1}*\frm{o}^2},
%
{(4,0)*+{1}\PATH ~={**\dir{-}}'(5,1)*+{2}^2},
{(3,1)*+{2}\PATH ~={**\dir{-}}'(4,2)*+{3}^1},
{(2,2)*+{3}\PATH ~={**\dir{-}}'(3,3)*+{4}^0},
{(1,3)*+{2}\PATH ~={**\dir{-}}'(2,4)*+{3}^2},
{(0,4)*+{1}\PATH ~={**\dir{-}}'(1,5)*+{2}^1},
%
{(6,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
           '(6,1)*+{2}*\frm{o}^2'(5,1)*+{2}*\frm{o}^0
		   '(5,2)*+{3}*\frm{o}^1'(4,2)*+{3}*\frm{o}^2
		   '(4,3)*+{4}*\frm{o}^0'(3,3)*+{4}*\frm{o}^1
		   '(3,4)*+{4}*\frm{o}^2'(2,4)*+{3}*\frm{o}^0
		   '(2,5)*+{3}*\frm{o}^1'(1,5)*+{2}*\frm{o}^2
		   '(1,6)*+{2}*\frm{o}^0'(0,6)*+{1}*\frm{o}^1},
%
{(6,0)*+{1}*\frm{o}\PATH ~={**\dir{.}}'(7,0)*+{}*\frm{}},
{(0,6)*+{1}*\frm{o}\PATH ~={**\dir{.}}'(0,7)*+{}*\frm{}},
%
{(6,1)*+{2}\PATH ~={**\dir{.}}'(7,2)*+{}*\frm{}},
{(5,2)*+{3}\PATH ~={**\dir{.}}'(6,3)*+{}*\frm{}},
{(4,3)*+{4}\PATH ~={**\dir{.}}'(5,4)*+{}*\frm{}},
{(3,4)*+{4}\PATH ~={**\dir{.}}'(4,5)*+{}*\frm{}},
{(2,5)*+{3}\PATH ~={**\dir{.}}'(3,6)*+{}*\frm{}},
{(1,6)*+{2}\PATH ~={**\dir{.}}'(2,7)*+{}*\frm{}},
%
\endxy
\bigskip fig. 5 \quad
%\medskip%\noindent
The beginning of the `Verma' support $\VV_{t_{-\lambda}}$ with 
multiplicities indicated in circles.
\bigskip
\vskip 1.5cm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig 6. of the `Verma' at translates of w_0
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
(-0.5,-0.5)*{w_0\,t_{-\lambda}},
%
{(0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,1)*+{2}*\frm{o}^0},
%
{(4,1)*+{2}*\frm{o}\PATH ~={**\dir{-}}
         '(3,0)*+{1}*\frm{o}^0'(2,0)*+{1}*\frm{o}^2
         '(2,1)*+{2}*\frm{o}^0'(1,1)*+{2}*\frm{o}^1
		 '(1,2)*+{2}*\frm{o}^2'(0,2)*+{1}*\frm{o}^0
		 '(0,3)*+{1}*\frm{o}^1'(1,4)*+{2}*\frm{o}^0},
%
{(2,1)*+{2}*\frm{o}\PATH ~={**\dir{-}}'(3,2)*+{3}*\frm{o}^2},
{(1,2)*+{2}*\frm{o}\PATH ~={**\dir{-}}'(2,3)*+{3}*\frm{o}^1},
%
{(5,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
         '(5,1)*+{2}*\frm{o}^0'(4,1)*+{2}*\frm{o}^1
         '(4,2)*+{3}*\frm{o}^2'(3,2)*+{3}*\frm{o}^0
		 '(3,3)*+{4}*\frm{o}^1'(2,3)*+{3}*\frm{o}^2
		 '(2,4)*+{3}*\frm{o}^0'(1,4)*+{2}*\frm{o}^1
         '(1,5)*+{2}*\frm{o}^2'(0,5)*+{1}*\frm{o}^0 },
%
{(5,0)*+{1}\PATH ~={**\dir{.}}'(6,0)*+{}},
{(0,5)*+{1}\PATH ~={**\dir{.}}'(0,6)*+{}},
%
{(5,1)*+{2}\PATH ~={**\dir{.}}'(6,2)*+{}*\frm{}},
{(4,2)*+{3}\PATH ~={**\dir{.}}'(5,3)*+{}*\frm{}},
{(3,3)*+{4}\PATH ~={**\dir{.}}'(4,4)*+{}*\frm{}},
{(2,4)*+{3}\PATH ~={**\dir{.}}'(3,5)*+{}*\frm{}},
{(1,5)*+{2}\PATH ~={**\dir{.}}'(2,6)*+{}*\frm{}},
\endxy
\bigskip fig. 6 \quad
%\medskip %\noindent
The beginning of the `Verma' support $\VV_{w_0 t_{-\lambda}}$ with 
multiplicities in circles.
\bigskip

\vskip 1cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig 7. of the three `fundamentals'
\hbox{
\xy
0;<\hrt cm,-.5cm>:<-\hrt cm,-.5cm>::
{  (1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
  '(2,1)*+{2}*\frm{o}^0'(3,1)*+{1}*\frm{o}^1  },
{  (2,1)*+{2}*\frm{o}\PATH ~={**\dir{-}}
  '(2,2)*+{1}*\frm{o}_2  },  
(.5,-.5)*{w_0},
\endxy
\hskip 1.5cm
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{  (0,0)*{\bullet}\PATH ~={**\dir{-}}
  '(1,0)*{\bullet}^2'(2,1)*{\UNIT}^0
  '(3,1)*{\bullet}^1'(3,0)*{\bullet}^0 },
{  (2,1)*{\UNIT}\PATH ~={**\dir{-}}
  '(2,2)*{\bullet}^2'(3,3)*{\bullet}^1 },  
\endxy 
\hskip 1.5cm
\xy 
0;<\hrt cm,-.5cm>:<-\hrt cm,-.5cm>::
{  (0,0)*{\bullet}\PATH ~={**\dir{-}}
  '(1,0)*{\bullet}^1'(2,1)*{\UNIT}^0
  '(3,1)*{\bullet}^2'(3,0)*{\bullet}^0 },
{  (2,1)*{\UNIT}\PATH ~={**\dir{-}}
  '(2,2)*{\bullet}^1'(3,3)*{\bullet}^2 },  
\endxy 
} \bigskip
fig. 7. \quad The supports of the three `fundamentals'.


\vskip 1.5cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig 8. of the p=5 alcove  
\bigskip
\xy 
0;<-\hrt cm,.5cm>:<\hrt cm,.5cm>::
{(-2,-2)\PATH~={**\dir{--}}'(-1,-2)'(0,-1)'(1,-1)
               '(2,0)'(3,0)'(4,1)'(5,1)'(6,2)'(7,2)
			   '(8,3)'(9,3)'(10,4)'(10,5)'(9,5)'(9,6)
			   '(8,6)'(8,7)'(7,7)'(7,8)'(6,8)'(6,9)
			   '(5,9)'(5,10)'(4,10)'(3,9)'(3,8)'(2,7)
			   '(2,6)'(1,5)'(1,4)'(0,3)'(0,2)'(-1,1)
			   '(-1,0)'(-2,-1)'(-2,-2)},
%
{(8,4)*+{40}*\frm{o}  \PATH~={**\dir{-}}
   '(7,4) *+{14}*\frm{-} ^{1} '(7,5) *+{01}*\frm{o} ^{2} 
   '(6,5) *+{12}*\frm{-} ^{0} '(6,6) *+{22}*\frm{o} ^{1}
   '(5,6) *+{21}*\frm{-} ^{2} '(5,7) *+{10}*\frm{o} ^{0}
   '(4,7) *+{41}*\frm{-} ^{1} '(4,8) *+{04}*\frm{o} ^{2}},
{(7,4)*+{14}*\frm{-}\PATH~={**\dir{-}}'(6,3)*+{03}*\frm{o} ^{0}}, %%%
{(6,5)*+{12}*\frm{-}\PATH~={**\dir{-}}'(5,4)*+{21}*\frm{o} ^{2}}, %%%
{(5,6)*+{21}*\frm{-}\PATH~={**\dir{-}}'(4,5)*+{12}*\frm{o} ^{1}}, %%%
{(4,7)*+{41}*\frm{-}\PATH~={**\dir{-}}'(3,6)*+{30}*\frm{o} ^{0}}, %%%
%
{(0,-1)\PATH~={**\dir{--}}'(0,0)*+{00}*\frm{o}},
{(2,0)\PATH~={**\dir{--}}'(2,1)*+{13}*\frm{o}},
{(4,1)\PATH~={**\dir{--}}'(4,2)*+{20}*\frm{o}},
{(6,2)\PATH~={**\dir{--}}'(6,3)*+{03}*\frm{o}},
{(8,3)\PATH~={**\dir{--}}'(8,4)*+{40}*\frm{o}}, %%%
{(9,5)\PATH~={**\dir{--}}'(8,4)*+{40}*\frm{o}}, %%%
{(8,6)\PATH~={**\dir{--}}'(7,5)*+{01}*\frm{o}}, %%%
{(7,7)\PATH~={**\dir{--}}'(6,6)*+{22}*\frm{o}}, %%%
{(6,8)\PATH~={**\dir{--}}'(5,7)*+{10}*\frm{o}}, %%%
{(5,9)\PATH~={**\dir{--}}'(4,8)*+{04}*\frm{o}}, %%%
{(3,8)\PATH~={**\dir{--}}'(4,8)*+{04}*\frm{o}}, %%%
{(2,6)\PATH~={**\dir{--}}'(3,6)*+{30}*\frm{o}},
{(1,4)\PATH~={**\dir{--}}'(2,4)*+{02}*\frm{o}},
{(0,2)\PATH~={**\dir{--}}'(1,2)*+{31}*\frm{o}},
{(-1,0)\PATH~={**\dir{--}}'(0,0)*+{00}*\frm{o}},
%
{(-1,-1)\PATH~={**\dir{.}}'(9,4)'(4,9)'(-1,-1)},
{(-1,-1)\PATH~={**\dir{.}}'(0,-2)},
{(-1,-1)\PATH~={**\dir{.}}'(-2,-3)},
{(-1,-1)\PATH~={**\dir{.}}'(-2,0)},
{(-1,-1)\PATH~={**\dir{.}}'(-3,-2)},
{(7,3) \PATH~={**\dir{.}}'(9,4)},
{(3,7) \PATH~={**\dir{.}}'(4,9)},
{(3,10)\PATH~={**\dir{.}}'(4,9)},
{(9,4) \PATH~={**\dir{.}}'(10,3)},
{(10,6)\PATH~={**\dir{.}}'(8,2)},
{(2,8) \PATH~={**\dir{.}}'(6,10)},
{(5,11)\PATH~={**\dir{.}}'(4,9)},
{(9,4) \PATH~={**\dir{.}}'(11,5)},
%
{(0,0)*+{00}*\frm{o} \PATH ~={**\dir{-}}
                '(1,1)*+{11}*\frm{-}^0},
%
{(2,1)*+{13}*\frm{o}\PATH ~={**\dir{-}}
'(1,1)*+{11}*\frm{-}^1'(1,2)*+{31}*\frm{o}^2},
%
{(2,1)*+{13}*\frm{o}\PATH ~={**\dir{-}} '(3,2)*+{31}*\frm{-}^2},
{(1,2)*+{31}*\frm{o}\PATH ~={**\dir{-}} '(2,3)*+{13}*\frm{-}^1},
%
{(4,2)*+{20}*\frm{o}\PATH ~={**\dir{-}} '(3,2)*+{31}*\frm{-}^0
'(3,3)*+{11}*\frm{o}^1'(2,3)*+{13}*\frm{-}^2'(2,4)*+{02}*\frm{o}^0},
%
{(4,2)*+{20}*\frm{o}\PATH ~={**\dir{-}} '(5,3)*+{32}*\frm{-}^1},
{(3,3)*+{11}*\frm{o}\PATH ~={**\dir{-}} '(4,4)*+{22}*\frm{-}^0},
{(2,4)*+{02}*\frm{o}\PATH ~={**\dir{-}} '(3,5)*+{23}*\frm{-}^2},
%
{(6,3)*+{03}*\frm{o}\PATH ~={**\dir{-}} '(5,3)*+{32}*\frm{-}^2
'(5,4)*+{21}*\frm{o}^0'(4,4)*+{22}*\frm{-}^1
'(4,5)*+{12}*\frm{o}^2'(3,5)*+{23}*\frm{-}^0
'(3,6)*+{30}*\frm{o}^1},
%
\endxy\bigskip 
fig. 8. \quad
The $p=5$ alcove.
% the dotted lines serving as borders are from the dual lattice; 
% reflecting in them gives the KW action; the weights $[n,m]$ are in
% circles, the weights $[[n,m]]$ in boxes

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 9. `exponents' in the p=5 case
\xy
0;<\hrt cm,.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{\bt}*\frm{o}\PATH ~={**\dir{-}}
'(1,0)*+{\bt}*\frm{o}'(2,0)*+{\bt}*\frm{o}
'(1,1)*+{\bt}*\frm{o}'(0,2)*+{\bt}*\frm{o}
'(0,1)*+{\bt}*\frm{o}'(0,0)*+{\bt}*\frm{o}},
%
{(3,3)*+{\bt}*\frm{o}\PATH ~={**\dir{-}}
'(3,2)*+{\bt}*\frm{o}'(3,1)*+{\bt}*\frm{o}
'(2,2)*+{\bt}*\frm{o}'(1,3)*+{\bt}*\frm{o}
'(2,3)*+{\bt}*\frm{o}'(3,3)*+{\bt}*\frm{o}},
%
{(3,0)*+{\bt}*\frm{o}\PATH ~={**\dir{.}}
'(2,1)*+{\bt}*\frm{o}'(1,2)*+{\bt}*\frm{o}'(0,3)*+{\bt}*\frm{o}},
%
{(4,0)*+{\bt}*\frm{o}\PATH ~={**\dir{.}}
'(4,1)*+{\bt}*\frm{o}'(4,2)*+{\bt}*\frm{o}'(4,3)*+{\bt}*\frm{o}
'(4,4)*+{\bt}*\frm{o}'(3,4)*+{\bt}*\frm{o}'(2,4)*+{\bt}*\frm{o}
'(1,4)*+{\bt}*\frm{o}'(0,4)*+{\bt}*\frm{o}},
%
{(6,0) \PATH ~={**\dir{-}}' (4,0)*+{\bt}'(3,0)*+{\bt}
'(2,0)*+{\bt}'(1,0)*+{\bt}'(0,0)*+{\bt}'(0,1)*+{\bt}
'(0,2)*+{\bt}'(0,3)*+{\bt}'(0,4)*+{\bt}'(0,6)},
%
(4.1,-.7)*{(0,p-1)},(-.7,4.1)*{(p-1,0)},(-.5,-.5)*{(0,0)},
%
(.6,.6)*{P^{p-3}_+}
\endxy
\vskip 1cm \bigskip
fig. 9a. \quad The dual set $E_p$ for $p=5$.

\vskip 1cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 9'. `exponents' in the p=4 case
\xy
0;<\hrt cm,.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{\bt}*\frm{o} \PATH ~={**\dir{-}}
'(0,1)*{\bt}*+\frm{o}'(0,2)*+{\bt}*\frm{o}'(0,3)*+{\bt}*\frm{o}
'(0,4)*{\bt}'(0,5)*{\bt}'(0,6)*{\bt}'(0,7)*{\bt}'(0,8)*{\bt}
'(0,9)*{\bt}'(1,8)*{\bt}'(2,7)*{\bt}'(3,6)*{\bt}'(4,5)*{\bt}
'(5,4)*{\bt}'(6,3)*{\bt}'(7,2)*{\bt}'(8,1)*{\bt}'(9,0)*{\bt}
'(8,0)*{\bt}'(7,0)*{\bt}'(6,0)*{\bt}'(5,0)*{\bt}'(4,0)*{\bt}
'(3,0)*+{\bt}*\frm{o}'(2,0)*+{\bt}*\frm{o}'(1,0)*+{\bt}*\frm{o}
'(0,0)*+{\bt}*\frm{o} },
%
{(2,2)*+{\bt}*\frm{o} \PATH ~={**\dir{-}}
'(2,1)*{\bt}*+\frm{o}'(1,2)*+{\bt}*\frm{o}'(2,2)*+{\bt}*\frm{o} },
%
{(0,1)*+{\bt}*\frm{o} \PATH ~={**\dir{-}}
'(1,0)*{\bt}*+\frm{o} },
%
(1,1)*+{\bt}*\frm{o},
(3,1)*+{\bt}*\frm{o},(3,2)*+{\bt}*\frm{o},(3,3)*+{\bt}*\frm{o},
(2,3)*+{\bt}*\frm{o},(1,3)*+{\bt}*\frm{o},
%
( 4,-2);(-2, 4)*++!U{H^{(p)}_\theta} **@{.},
(-1,-2)*++!DR{H^{(0)}_{\alpha_2}};(-1,11) **@{.},
(-2,-1)*++!UR{H^{(0)}_{\alpha_1}};(11,-1) **@{.},
(-1,11);(11,-1) **@{.},
(-2,8)*++!U{H^{(2p)}_\theta};(8,-2) **@{.},
(-2,7)*++!UR{H^{(2p)}_{\alpha_1}};(4,7) **@{.},
(7,4);(7,-2)*++!DR{H^{(2p)}_{\alpha_2}} **@{.},
(-2,3)*++!UR{H^{(p)}_{\alpha_1}};(8,3) **@{.},
(3,8);(3,-2)*++!DR{H^{(p)}_{\alpha_2}} **@{.},
%
(7,1)*{\bt},(6,2)*{\bt},(5,3)*{\bt},(4,4)*{\bt},(3,5)*{\bt},
(2,6)*{\bt},(1,7)*{\bt},(1,6)*{\bt},(2,5)*{\bt},(3,4)*{\bt},
(4,3)*{\bt},(5,2)*{\bt},(6,1)*{\bt},(5,1)*{\bt},(4,2)*{\bt},
(2,4)*{\bt},(1,5)*{\bt},(1,4)*{\bt},(4,1)*{\bt},
%
(0.1,0.1)*+!L{P^{1}_+}
\endxy
\vskip 1cm \bigskip
fig. 9b. \quad The dual set $E_p\subset P^{3p-3}_+$ for the case $p=4$.
\bye

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 9. `exponents' in the p=5 case
\xy
0;<\hrt cm,.5cm>:<\hrt cm,-.5cm>::
{(0,0)*{\bt}\PATH ~={**\dir{-}}
'(1,0)*{\bt}'(2,0)*{\bt}'(1,1)*{\bt}'(0,2)*{\bt}
'(0,1)*{\bt}'(0,0)*{\bt}},
%
{(3,3)*{\bt}\PATH ~={**\dir{-}}
'(3,2)*{\bt}'(3,1)*{\bt}'(2,2)*{\bt}'(1,3)*{\bt}
'(2,3)*{\bt}'(3,3)*{\bt}},
%
{(3,0)*+{\st}\PATH ~={**\dir{--}}
'(2,1)*+{\st}'(1,2)*+{\st}'(0,3)*+{\st}},
%
{(4,0)*+{\st}\PATH ~={**\dir{--}}
'(4,1)*+{\st}'(4,2)*+{\st}'(4,3)*+{\st}
'(4,4)*+{\st}'(3,4)*+{\st}'(2,4)*+{\st}
'(1,4)*+{\st}'(0,4)*+{\st}},
%
{(6,0) \PATH ~={**\dir{=}}' (4,0)*+{\st}'(3,0)*+{\st}
'(2,0)*+{\bt}'(1,0)*+{\bt}'(0,0)*+{\bt}'(0,1)*+{\bt}
'(0,2)*+{\bt}'(0,3)*+{\st}'(0,4)*+{\st}'(0,6)},
%
(4.1,-.7)*{(p-1,0)},(-.7,4.1)*{(0,p-1)},(-.5,-.5)*{(0,0)},
%(0,0)*{A},(1,0)*{B},(0,1)*{C},
\endxy
\vskip 1cm \bigskip
fig. 9. \quad The dual set $E_p$ for $p=5$.


\vskip 2cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fig. 9'b. comparison with i(W)  in the p=4 case
\xy
0;<\hrt cm,.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{\bt}*\frm{o} \PATH ~={**\dir{-}}
'(0,1)*{\bt}'(0,2)*{\bt}'(0,3)*+{\bt}*\frm{o}
'(0,4)*{\bt}'(0,5)*{\bt}'(0,6)*+{\bt}*\frm{o}'(0,7)*{\bt}'(0,8)*{\bt}
'(0,9)*{\bt}*+\frm{o}'(1,8)*{\bt}'(2,7)*{\bt}'(3,6)*{\bt}*+\frm{o}'(4
,5)*{\bt}
'(5,4)*{\bt}'(6,3)*{\bt}*+\frm{o}'(7,2)*{\bt}'(8,1)*{\bt}'(9,0)*{\bt}
*+\frm{o}
'(8,0)*{\bt}'(7,0)*{\bt}'(6,0)*+{\bt}*\frm{o}'(5,0)*{\bt}'(4,0)*{\bt}
'(3,0)*+{\bt}*\frm{o}'(2,0)*{\bt}'(1,0)*{\bt}
'(0,0)*+{\bt}*\frm{o} },
%
{(0,9)*+{\bt}*\frm{o} \PATH ~={**\dir{--}}
'(1,7)*{\bt}*+\frm{o}'(3,6)*+{\bt}*\frm{o}'(4,4)*+{\bt}*\frm{o} 
'(6,3)*{\bt}*+\frm{o}'(7,1)*+{\bt}*\frm{o}'(9,0)*+{\bt}*\frm{o} },
%
{(1,7)*+{\bt}*\frm{o} \PATH ~={**\dir{--}}
'(0,6)*{\bt}*+\frm{o}'(1,4)*+{\bt}*\frm{o}'(3,3)*+{\bt}*\frm{o} 
'(4,1)*{\bt}*+\frm{o}'(6,0)*+{\bt}*\frm{o}'(7,1)*+{\bt}*\frm{o} },
%
{(3,3)*+{\bt}*\frm{o} \PATH ~={**\dir{--}}'(4,4)*{\bt}*+\frm{o}},
%
{(1,4)*+{\bt}*\frm{o} \PATH ~={**\dir{--}}
'(0,3)*{\bt}*+\frm{o}'(1,1)*+{\bt}*\frm{o}'(3,0)*+{\bt}*\frm{o} 
'(4,1)*{\bt}*+\frm{o}},
%
{(0,0)*+{\bt}*\frm{o} \PATH ~={**\dir{--}}'(1,1)*{\bt}*+\frm{o}},
%
(6,2)*{\bt},(5,3)*{\bt},(3,5)*{\bt},(2,6)*{\bt},
(1,6)*{\bt},(2,5)*{\bt},(3,4)*{\bt},
(4,3)*{\bt},(5,2)*{\bt},(6,1)*{\bt},
(5,1)*{\bt},(4,2)*{\bt},(2,4)*{\bt},(1,5)*{\bt},
(2,3)*{\bt},(3,2)*{\bt},
(1,3)*{\bt},(2,2)*{\bt},(3,1)*{\bt},
(1,2)*{\bt},(2,1)*{\bt},
\endxy
\vskip 1cm \bigskip
fig. 9b. \quad The sets 
              $\iota({\cal W}^{(+)}_p)\subset P^{3p}_+$ 
			  for the case $p=4$.

\bye

\hbox{
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{  (0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
  '(1,0)*+{1}*\frm{o}^2'(2,1)*+{1}*\frm{o}^0
  '(3,1)*+{1}*\frm{o}^1'(3,0)*+{1}*\frm{o}^0 },
{  (2,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}
  '(2,2)*+{1}*\frm{o}^2'(3,3)*+{1}*\frm{o}^1 },  
\endxy 
\hskip 1.5cm
\xy 
0;<\hrt cm,-.5cm>:<-\hrt cm,-.5cm>::
{  (0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
  '(1,0)*+{1}*\frm{o}^1'(2,1)*+{1}*\frm{o}^0
  '(3,1)*+{1}*\frm{o}^2'(3,0)*+{1}*\frm{o}^0 },
{  (2,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}
  '(2,2)*+{1}*\frm{o}^1'(3,3)*+{1}*\frm{o}^2 },  
\endxy 
}




\bye

\hbox{
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{  (0,0)*{\bullet}\PATH ~={**\dir{-}}
  '(1,0)*{\bullet}^2'(2,1)*{\bullet}^0
  '(3,1)*{\bullet}^1'(3,0)*{\bullet}^0 },
{  (2,1)*{\bullet}\PATH ~={**\dir{-}}
  '(2,2)*{\bullet}^2'(3,3)*{\bullet}^1 },  
\endxy 
\hskip 1.5cm
\xy 
0;<\hrt cm,-.5cm>:<-\hrt cm,-.5cm>::
{  (0,0)*{\bullet}\PATH ~={**\dir{-}}
  '(1,0)*{\bullet}^1'(2,1)*{\bullet}^0
  '(3,1)*{\bullet}^2'(3,0)*{\bullet}^0 },
{  (2,1)*{\bullet}\PATH ~={**\dir{-}}
  '(2,2)*{\bullet}^1'(3,3)*{\bullet}^2 },  
\endxy 
}

\bye


